New minimal, median, and maximal propagation models for dark matter searches with Galactic cosmic rays

Galactic charged cosmic rays (notably electrons, positrons, antiprotons and light antinuclei) are powerful probes of dark matter annihilation or decay, in particular for candidates heavier than a few MeV or tiny evaporating primordial black holes. Recent measurements by PAMELA, AMS-02, or VOYAGER on positrons and antiprotons already translate into constraints on several models over a large mass range. However, these constraints depend on Galactic transport models, in particular the diffusive halo size, subject to theoretical and statistical uncertainties. We update the so-called MIN-MED-MAX benchmark transport parameters that yield generic minimal, median and maximal dark-matter induced fluxes; this reduces the uncertainties on fluxes by a factor of about 2 for positrons and 6 for antiprotons, with respect to their former version. We also provide handy fitting formulae for the associated predicted secondary antiproton and positron background fluxes. Finally, for more refined analyses, we provide the full details of the model parameters and covariance matrices of uncertainties.

==> Tex/stat_method_old.tex <==
% Laurent, David, Yoann
% Please use \citefig{} \citetab{} etc. defined in newcommands.tex
%
\section{Statistical method}
\label{sec:stats}

In this section, we describe the method used to derive the parameters corresponding the \min{}, \med{} and \max{} model.
To illustrate the method, we use the \slim{} model and the results obtained in \cite{WeinrichEtAl2020b} from
the combined analysis of Li/C, B/C and Be/B data from AMS02 and $^{10}$Be/Be+$^{10}$Be/$^9$Be data from
previous experiments (see Table~2 of \cite{WeinrichEtAl2020b}). The covariance matrix for propagation parameters is
derived from the Hessian matrix obtained from \migrad{} algorithm of the \minuit{} package~\cite{JamesEtAl1975} rescaled with error obtained from the \minos{} algorithm.
Assuming that the parameters are distributed as a multidimensional Gaussian, the covariance matrix and the best fit values are used to draw $N=10^5$ samples of propagation model parameters. 

Fig. \ref{fig:stat_KR} shows the diffusion coefficients $K(R)$ (see Eq.~\ref{eq:def_K}) and the ratio $L^2/K(R)$ as a function of rigidity $R$ computed for a few hundreds of the $N$ samples.

\begin{figure}[h]
  \includegraphics[width=0.9\columnwidth]{K_L2overK_2sig}
    \caption{Diffusion coefficients $K(R)$ (top) and the ratio $L^2/K(R)$ (bottom) as a function of rigidity $R$ computed for a few hundreds of the $N$ samples are shown as solid blue lines.
    Orange lines show the $K(R)$ (top) and the ratio $L^2/K(R)$ (bottom) as a function of $R$ obtained for the 2$sigma$ ($n=2$) \min-\med-\max{} models (dashed-solid-dotted lines resp.).}
  \label{fig:stat_KR}
\end{figure}

Fig. \ref{fig:stat_KR_dist} shows the distribution obtained from $N=10^5$ samples of the quantity
$\log_{10} \left( L^2/K(R) \right)$ for $R=10$~GV .  To define the \min{}, \med{}, \max{} models from this distribution, we select subsamples of models for which
$$ q_{X} - \frac{p}{2} < \log_{10} \left( L^2/K(R=10\, \mathrm{GV}) \right) < q_{X}+\frac{p}{2}$$
where $X$ stands for \min{}, \med{}, \max{}. Here $p$ is the width of the quantile interval and should be chosen to get enough statistics in each subsample and the $q_X$ are given by~: 
\ben
q_{\textrm{\min{}}}  & = & \frac{1}{2} \left(1 - \mathrm{erf} \left(\frac{n}{\sqrt{2}}\right) \right) \nn\\
q_{\textrm{\med{}}}  & = & .5 \nn\\
q_{\textrm{\max{}}}  & = & \frac{1}{2} \left(1 + \mathrm{erf} \left(\frac{n}{\sqrt{2}}\right) \right)  \nn
\een
where $\mathrm{erf}(x) = 2/\sqrt{\pi}\int_{-\infty}^x e^{-t^2}\mathrm{d} t$ is the error function and $n=1, 2, \ldots$ define $n\sigma$ \min{} and \max{} models.
Fig. \ref{fig:stat_KR_dist} shows the distribution of $  \log_{10} \left( L^2/K(R=10 \,\mathrm{GV}) \right) $  for the \min{}, \med{}, \max{} subsamples obtained for $n=1$ and $n=2$ with $p=0.01$.

\begin{figure}[!h]
  \includegraphics[width=0.9\columnwidth]{K_L2overK_dist}
    \caption{Distribution of  $  \log_{10} \left( L^2/K(R=10 \,\mathrm{GV}) \right) $ for the full
    sample (blue histogram) and for the 1$\sigma$ and 2$\sigma$ (resp. green and red histograms) subsamples used to define \min-\med-\max{}.  }
  \label{fig:stat_KR_dist}
\end{figure}

The distribution of parameter values for the full sample and  2$\sigma$ \min-\med-\max{} subsamples are shown on Fig.~\ref{fig:stat_pars}. As expected, \min, \max{} models have respectively 
lower, larger $L$ values and due to the strong $K_0$-$L$ correlation respectively larger, lower $K_0$ values. Subsamples distribution for other parameters are close to the one obtained for the full sample.  
\begin{figure}[!h]
  \includegraphics[width=0.8\columnwidth]{par_dist_2sig}
  \caption{Distribution of propagation parameter values for the full sample of
    models (All) and for the subsamples corresponding to \min-\med-\max{} width $n=2$ and for $R = 10$~GV}
  \label{fig:stat_pars}
\end{figure}

Finally the propagation parameters corresponding to \min{}, \med{}, \max{} are
then computed by taking the average values on each corresponding subsample. The 1 and 2 $\sigma$ 
propagation parameters obtained for \min{}, \med{} and \max{} are displayed on Tab.~\ref{tab:stat_parvalues}. 

\begin{table}[!h]                                                       
\begin{tabular}{p{1.2cm}|p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}}
     1$\sigma$    &   $\log_{10} L$ &   $\delta$ &   $\log_{10} K_0$ &   $R_\mathrm{low}$ &   $\delta_\mathrm{low}$ \\

\hline
 \max        &           0.775 &      0.498 &            -1.342 &              4.511 &                   1.087 \\
 \med        &           0.669 &      0.500 &            -1.444 &              4.484 &                   1.101 \\
 \min        &           0.564 &      0.500 &            -1.542 &              4.460 &                   1.130 \\
\hline
\end{tabular} 

    \vspace{.3cm}
\begin{tabular}{p{1.2cm}|p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}p{1.2cm}}

     2$\sigma$    &   $\log_{10} L$ &   $\delta$ &   $\log_{10} K_0$ &   $R_\mathrm{low}$ &   $\delta_\mathrm{low}$ \\
\hline
 \max        &           0.879 &      0.497 &            -1.244 &              4.519 &                   1.073 \\
 \med        &           0.669 &      0.500 &            -1.444 &              4.484 &                   1.101 \\
 \min        &           0.457 &      0.502 &            -1.644 &              4.441 &                   1.144 \\
\hline

\end{tabular} 
    \caption{Propagation parameters for 1$\sigma$ and 2$\sigma$ \min{}-\med{}-\max{} models}
    \label{tab:stat_parvalues}
\end{table}


%\subsection{}
%\label{ssec:}
%\subsubsection{}
%\label{sssec:}

